Online Learning with Pairwise Loss Functions

Efficient online learning with pairwise loss functions is a crucial component in building large-scale learning system that maximizes the area under the Receiver Operator Characteristic (ROC) curve. In this paper we investigate the generalization performance of online learning algorithms with pairwise loss functions. We show that the existing proof techniques for generalization bounds of online algorithms with a univariate loss can not be directly applied to pairwise losses. In this paper, we derive the first result providing data-dependent bounds for the average risk of the sequence of hypotheses generated by an arbitrary online learner in terms of an easily computable statistic, and show how to extract a low risk hypothesis from the sequence. We demonstrate the generality of our results by applying it to two important problems in machine learning. First, we analyze two online algorithms for bipartite ranking; one being a natural extension of the perceptron algorithm and the other using online convex optimization. Secondly, we provide an analysis for the risk bound for an online algorithm for supervised metric learning.

==> texfiles/discuss.tex <==
\section{Related Work}
\label{sec:discuss}
Several theoretical studies investigated the batch setting.
\cite{freund2003efficient}
gave generalization bounds for the RankBoost algorithm, based on
the uniform convergence results for classification.
\cite{agarwal2005generalization} derived uniform convergence bounds for the
bipartite ranking loss, using a quantity called rank-shatter coefficient, which
generalizes ideas from the classification setting.
Agarwal et.\ al.\
%\cite{agarwal2005stability}
provided bounds for the bipartite ranking
problem \citep{agarwal2005stability} and the general ranking problem
\citep{agarwal2009generalization} using ideas from
algorithmic stability.
\cite{rudin2005margin} approached a closely related problem where the goal is
to correctly rank only the top of the ranked list, and derived generalization
bounds based on $L_\infty$ covering number.
Recently, several authors investigated
oracle inequalities for pairwise-based quantities via the formalization of $U$-statistics
\citep{clemencon2008ranking, rejchel2012ranking} using empirical processes. \cite{peel2010empirical} gave an empirical Bernstein inequality for higher order $U$-statistics.

Another thread comes from the perspective of reducing ranking problems to the more familiar classification problems. For the bipartite ranking problem, \cite{kotllowski2011bipartite} provided a upper bound on the ranking risk in terms of risk that is obtained using several univariate loss function, e.g. 0-1 loss, logistic loss, margin loss, etc. We consult interested readers to the following references. 

==> texfiles/notes.tex <==
\section{Notes}

In general, we never need Theorem 16, which is the buffer based version of Theorem 1. From my point of view, the process should be as follows,\\

Recall the sample statistics as
\begin{equation}
\label{eqn:mn}
\begin{split}
\M^n(Z^n) = \nmlz M_t(Z^t),\qquad M_t(Z^t) =
\frac{1}{t-1}\sum_{i=1}^{t-1} \ell\left(h_{t-1}, \z_t, \z_i\right),
\end{split}
\end{equation}
where $c_n = \lceil c\cdot n \rceil$ and $c\in(0,1)$ is a small
positive constant. 

Our theorem says that from the ensemble $H=\{h_1, \cdots, h_n\}$, we can find $\hat{h}$ such that
\[
\Pr(\R(\hat{h}) \geqslant \M^n + \epsilon) \leqslant \delta.
\] 
Thus, all we need to do is find an online learning algorithm that achieves low error $\M^n$. For the infinite buffer algorithm, we can have garantees on $\M^n$, but we are saying that this is too costly. We want some algorithm that we can bound the number of iterations of the inner loop. Therefore, we come up with buffer based algorithms that optimize an another statistic $\M_B^n$, which is shown to be upper bounded by $\M_B^*$, our hope is that optimizing $\M_B^n$ amounts to optimizing $\M^n$. Thus, we want $\M_B^*$ is also an upper of $\M^n$ (maybe probabilistically). \\

\textbf{Question:} We want to design a buffer based algorithm $\mathcal{A}_B$ such that
\begin{itemize}
  \item At each iteration, the computational complexity is $\mathcal{O}(1)$.
  \item Suppose $\mathcal{A}_B$ achieves error $\M^n_B$ that is bounded by $\M_B^*$, we want
  \[    
    \Pr(\M^n \geqslant \M^n_B + \epsilon) \leqslant \delta,
  \]
  which essentially yields
  \[
   \Pr(\M^n \geqslant \M^*_B + \epsilon) \leqslant \delta
  \]
\end{itemize} 
Of course, we need a good buffer strategy to make sure $\M^n_B$ is close to $\M^n$. Consequently, the question broils down to the following: can we prove, for $\mathcal{A}_B$ such that
\[
\Pr(\R(\hat{h}) \geqslant \M^*_B + \epsilon) \leqslant \delta.
\] 
Notice that on the right hand side it is $\M^*_B$ instead of $\M^*$. Hence, I'd say we need a bound as the one in~\cite{zhao2011online}, not the buffered based generalization bound as Theorem 16. 

